Scene-level Pose Estimation for Multiple Instances of Densely Packed Objects

This paper introduces key machine learning operations that allow the realization of robust, joint 6D pose estimation of multiple instances of objects either densely packed or in unstructured piles from RGB-D data. The first objective is to learn semantic and instance-boundary detectors without manual labeling. An adversarial training framework in conjunction with physics-based simulation is used to achieve detectors that behave similarly in synthetic and real data. Given the stochastic output of such detectors, candidates for object poses are sampled. The second objective is to automatically learn a single score for each pose candidate that represents its quality in terms of explaining the entire scene via a gradient boosted tree. The proposed method uses features derived from surface and boundary alignment between the observed scene and the object model placed at hypothesized poses. Scene-level, multi-instance pose estimation is then achieved by an integer linear programming process that selects hypotheses that maximize the sum of the learned individual scores, while respecting constraints, such as avoiding collisions. To evaluate this method, a dataset of densely packed objects with challenging setups for state-of-the-art approaches is collected. Experiments on this dataset and a public one show that the method significantly outperforms alternatives in terms of 6D pose accuracy while trained only with synthetic datasets.

==> 04_hg.tex <==
The previous step outputs per-pixel and semantic class predictions
$\segnet$ and boundary prediction $\boundarynet$\footnote{The
following discussion drops the term $x$ from $\boundarynet(.|x)$ and
$\segnet(.|x)$ as the computations for generating hypotheses operate
over a single image.}.  Given these predictions, this step aims to
generate a set of 6D pose hypotheses
$\{\{\trans_{ij} \}_{j=1}^{H_i} \}_{i=1}^{K}$, where $H_i$ denotes the
number of pose hypotheses for each object model $M_i$ and is larger
than the number of the object's instances in the scene, i.e, $H_i \gg
N_i$. Similar to the overall objective of the problem setup, each
$T_{ij} = (t_{ij}, R_{ij})$ is a candidate translation $t_{ij} \in
R^3$ and rotation $R_{ij} \in SO(3)$ of some instance of object type
$\model_i$ in the camera's reference frame, for each of the $K$ object
types present in the scene.

The sets of pose hypotheses should be sufficiently large to ensure
they contain candidates close enough to the unknown true poses, i.e,
$$\forall i \in [1, K],\forall j \in [1,N_i], \exists\
T \in \{\trans_{ij'} \}_{j'=1}^{H_i} : \| \trans
- \trans^g_{ij}\|\leq \epsilon,$$ where $\trans$
is a hypothesis pose for object $M_i$ and $\trans^g_{ij}$ is the
ground truth pose of the $j^{th}$ instance of object $M_i$.  Since the
ground truth poses are unknown during testing, one cannot guarantee
that the previous desired property will be satisfied unless the
candidates are densely sampled from $SE(3)$, which would make the
search computationally expensive.  Therefore, it is important to
sample the candidates in a manner that balances their diversity and
their similarity to the ground truth given the semantic class
predictions $\segnet$ and models $\{M_i\}_{i=1}^{K}$.

Pose hypotheses generation is often performed using RANSAC-like
techniques~\cite{brachmann2014learning} or via hough
voting~\cite{drost2010model}, or various distinctive geometric
features~\cite{hinterstoisser2016going,mitash2018robust,michel2017global},
which ensure that multiple points can be sampled from the same
object. These methods do not incorporate boundary information, which
is important in cases where the surfaces of multiple object instances
are aligned. The following explains the proposed pose hypotheses
generation process, which utilizes both semantic segmentation and
instance-boundaries.


% \begin{wrapfigure}{r}{1.5in}
%   \centering \includegraphics[width=1.45in]{images/HG1}
% \caption{Hypothesis generation process via sampling a base and
%   matching it to a congruent set from the object model.}
%   \label{fig:qualitative}
% \end{wrapfigure}

The output of the softmax layer from $\segnet$ is used to compute
$\pi_{l} (\pixel_i)$, the probability of each pixel $\pixel_i$
belonging to an object class $l$. This probability is defined as the
ratio of the output $\segnet(\pixel_i)$ over the sum of the outputs
for the same class over all pixels $\pixel$ in the given test image
$x$, i.e./ $\pi_{l} (\pixel_i)
= \frac{\segnet(\pixel_i)}{\sum_{\pixel}\segnet(\pixel)}.$

Based on the principles of randomized alignment, candidate poses are
generated for each instance of an object by sampling sets of points
that belong to one instance with high probability.  In the point cloud
registration literature \cite{mellado2014super, Huang:2017aa}, a set
of sampled points is called a {\it base} and denoted by $\base$.  Once
sampled, this set is matched to {\it congruent} sets, denoted by $U$,
on the corresponding object model $M$. Each of the congruent pairs
$(B,U)$ defines a unique rigid transform as long as both $B$ and $U$
contain at least 3 points each. For computational reasons, the
cardinality is typically limited to 4, i.e., $|\base| = |U| = 4$. To
maximize the probability that pose candidates for all the instances
are generated, a number $A_i$ of base sets $\{B_{ij} \}_{j=1}^{A_i}$
on the image $x$ is sampled, for each object class $i \in \{1, \dots,
K\}$. Each base $B_{ij}$ can be matched to several congruent bases $U$
on the models, and thus defines a large set of candidate poses.

%We first explain how the bases are sampled, then show how the bases
%are transformed into poses.


%The first point, $b_{1}$ is always directly sampled from the prior $\pi_l$. The selection of the first point restricts the object instance that the other samples need to come from. Thus,

\emph{A. Sampling a Base from a Single Object Instance:}
The four 3D points that form a base $\base = \{b_{1}, b_{2}, b_{3},
b_{4} \mid b_{1:4} \in S_l\}$ are sampled from a point cloud $S_l$,
which is the set of 3D points that are labeled as a category $l$
according to the semantic class probabilities $\segnet$.  The
challenge here is to maximize the joint probability of the four points
belonging to the same object instance. The joint probability
distribution on the graph formed by the four points is represented by
using the Hammersley-Clifford factorization and considering only unary
and binary relations between the points:

\begin{eqnarray}
	Pr\Big( \big( c(p(b_1),x) = l \big) \wedge \big(b_{1:4} \textrm{ are all on the same instance}\big)\Big)  \nonumber \\ = \frac{1}{Z}
\prod_{i=1}^{4} \Big( \potential^{l}_{node}(b_i) \prod_{j=1}^{j<i} \potential^{l}_{edge}(b_i,b_j) \Big), \nonumber
\end{eqnarray}

\noindent where $p(b_i)$ is used to denote the pixel corresponding to the 3D
point $b_i$ and, as before, $c(p,x)$ is used to denote the object
class label of pixel $p$ in image $x$. The unary terms
$\potential^{l}_{node}(b_i)$ are the individual probabilities of
labeling pixels $p(b_i)$ with category label $l$, i.e.,
$\potential^{l}_{node}(b_i) = \segnet(p(b_i))$. The binary relations
are defined as,

\begin{eqnarray*}
	\potential^{l}_{edge}(b_i, b_j) = 
	\begin{cases}
	1, & \text{ if } {\tt PPF}(b_i,b_j) \in {\tt PPF}(M_k) \text{ and} \cr
	   & \textrm{ \it \small length-of-shortest-path}(p(b_i),p(b_j)) < \epsilon_l \cr
	0, & \text{ otherwise}.
	\end{cases}
\end{eqnarray*}

The {\it Point-Pair Feature} ({\tt PPF}) \cite{drost2010model} for two
base points $b_i, b_j$ with surface normals $n_i, n_j$ is defined as:

\begin{align*}
	{\tt PPF}(b_i,b_j) = (\mid\mid d \mid\mid_2, \angle(n_i, d), \angle(n_j, d), \angle(n_i, n_j)),
\end{align*}

\noindent where $d=b_i-b_j$ is the vector from $b_i$ to $b_j$ and $n_i,
n_j$ are local surface normals.  ${\tt PPF}(M_k)$ is the set of
point-pair features pre-computed on the object model $M_k$ of object
category $k$. The \textrm {\it \small length-of-shortest-path} term is
the shortest distance on a graph $G$, where the vertices are the image
pixels and an edge connects two pixels $p_i$ and $p_j$ if and only if:
$P_B(p_i) < \delta$, $P_B(p_j) < \delta$, and $p_i$ and $p_j$ are
adjacent pixels in the image (each pixel has at most eight adjacent
pixels). In other terms, there is an edge between two adjacent pixels
if both pixels have a low probability (less than a threshold $\delta$)
of being on the boundary of an object. Thus, $\textrm{ \it \small
length-of-shortest-path}(p_i,p_j)$ is the length of the shortest path
between the two nodes on $G$, and it is obtained using a breadth-first
search.


\begin{comment}
\begin{align*}
G = \{P, E\}, \text{P is a set of all pixels in the image}
\end{align*}
\begin{align*}
E = \{(p_i, p_j) | p_i, p_j \in P, \\
	 P_B[p_i] < \delta, \\
	 P_B[p_j] < \delta, \\
	 p_i \in 8-NEIGHBOR(p_j)\}
\end{align*}
\end{comment}

\emph{B. Avoiding Oversampling and Achieving Coverage:}
The sampling process is dynamically adapted so as to avoid
repetitively selecting the same image regions. In particular, after a
base is sampled, a decay factor $\gamma\in[0,1)$ is multiplied to the
potential $\potential^{l}_{node}(b_i)$ of every point $b_i$ that
belongs to the same segment as $b_i$, i.e.,
$\potential^{l}_{node}(b_i)\leftarrow \gamma \potential^{l}_{node}(b_i)$. Points
belonging to the same segments are those encountered during the
breadth-first search. This encourages dispersion in the sampling
process of the bases, so as to cover all instances of objects in the
image and avoid having all the samples concentrated in the region of a
single object instance. This becomes an issue when a particular, more
prominent object instance has higher semantic class prediction
probability than other instances.

%The four points of the base can be represented by two pairs represented by their respective PPF, the ratio defined on the line segments and angle defined by virtue of their intersection~\textcolor{red}{(needs clarification)}. Two sets of point pairs are computed on the model with the PPFs specified by the segment base. The pairs in the two sets, which also intersect with the given ratios and have similar angles are classified as congruent 4-points. 

\emph{C. Matching the Base to its Congruent Sets:}
Once all the base sets are sampled, a matching process is used for
each one of the sampled bases $\{\{B_{ij} \}_{j=1}^{A_i} \}_{i=1}^{K}$
to compute a set $U_{ij}=\{u_1,u_2,u_3,u_4\}$ of 4-points from $M_i$
that are congruent to the sampled bases.  The basic idea of 4-point
congruent sets was derived from the fact that ratios and distances on
objects are invariant across any rigid
transformation~\cite{aiger20084}.

This matching process generates a large number of pose candidates
$\{\{\trans_{ij} \}_{j=1}^{H_i} \}_{i=1}^{K}$, several of which are
redundant due to different congruent pairs returning similar
transforms and the fact that most geometries have symmetry along
multiple axes. Thus, this work follows a greedy approach to provide a
diverse subset of the population. The approach sorts all pose
candidates based on the Largest Common Pointset
score~\cite{mellado2014super} and picks pose representatives that are
beyond a minimum distance from already selected poses. The distance
here takes into account symmetry, and there are separate thresholds
for rotation and translation, since these two variables operate in
different spaces. The resulting set
$\{\{\trans_{ij} \}_{j=1}^{H_i} \}_{i=1}^{K}$ of pose representatives
then undergoes local refinement using ICP.

\section{Pose Hypothesis Quality Evaluation}
\label{sec:hypeval}

%scoring each candidate based on several criteria. The scores are all
%related to the similarity between how the object would look like in
%the scene when placed according to its hypothesized pose and the
%portion of the image it would occupy according to that pose. Each
%score captures a different aspect of similarity, such as the overlap
%between surfaces and the overlap between boundaries.  To compute these
%similarity scores, the model is projected to the camera frame and the
%Z-buffer algorithm is used to obtain the depth map of the visible
%portion of the model at the given pose. The depth map is compared to
%the depth map obtained from the sensor to remove the portion of the
%model that is occluded by other objects. Finally, a Sobel filter is
%used to find the boundary of this visible portion of the depth map.

%We define these indicators here and explain later how they are
%combined to compute a single score $f(T)$ per candidate pose $T$. 


For each pose $T$ in the set of hypotheses
$\{\{\trans_{ij} \}_{j=1}^{H_i} \}_{i=1}^{K}$, a quality score
function $f(T)$ is computed.  The proposed score function considers
five indicators $f_{1:5}(T)$ of a good alignment for each pose
candidate $T$. The different scores $f_{1:5}(T)$ are automatically
combined into a single score $f(T)$.

\emph{A. Computing the Score from Component Indicators:} A
straightforward solution is to define $f$ as a weighted sum of its
components $f_{1:5}$. Nevertheless, the resulting poses would heavily
depend on the choice of the weights of the scores, and choosing the
right weights manually for every new type of objects is not trivial.
Instead, a key feature of the proposed pipeline is to learn the
objective function $f(T)$ using $f_{1:5}(T)$ as features. Namely,
$f(T)$ is defined as: $f(T) = h([f_{1}(T),f_{2}(T),
f_{3}(T),f_{4}(T),f_{5}(T) ])$.  The function $h$ is learned by
minimizing the following loss:

\begin{eqnarray}
\underset{h} {\textrm{min}} \sum_{(T,f_{1:5}(T),T^{g}) \in \mathcal T_{train}}  \Big( h(f_{1:5}(T)) -  e_{ADI}(T,T^g) \Big)^2,
\label{GBRT_obj}
\end{eqnarray}

\noindent where $e_{ADI}(T,T^g)$ is the distance between a given pose
$T$ and a ground-truth pose $T^g$. The distance $e_{ADI}(T,T^g)$ is
computed using the $ADI$ metric, which is frequently used in the
literature for evaluating pose
estimations~\cite{hinterstoisser2012model}. This metric is explained
in the experimental section.


\begin{figure}[t]
  \centering \includegraphics[width=\linewidth]{images/hypothesis_validation}
\caption{Regressing the hypothesis quality given various alignment features.}
  \label{fig:qualitative}
\end{figure}


The training data set $\mathcal T_{train}$ is collected by simulating
different scenes using the models of the objects in a physics engine.
Synthetic images are obtained by systematically generating random
ground-truth poses and rendering the models accordingly.  For each
instance of an object in the synthetic images, a number of random
poses $T$ is also generated so as to extract their score features
$f_{1:5}(T)$ and calculate the distances $e_{ADI}(T,T^g)$.  Clearly,
$e_{ADI}(T,T^g)$ can be computed only for training data, because $T^g$
is unknown in the test data.  The regression learning problem here
consists in finding a function $h$ that maps score features
$f_{1:5}(T)$ of a pose $T$ to its actual distance from the
corresponding ground-truth pose $T^g$.

This work adopts the Gradient Boosted Regression Trees (GBRT) to solve
the optimization problem in Equation~\ref{GBRT_obj}. GBRTs are
well-suited from handling variables that have heterogeneous
features~\cite{elith2008working}. GBRTs are also a flexible
non-parametric approach that can adapt to non-smooth changes in the
regressed function using limited data, which often occurs when dealing
with objects that have different shapes and sizes. An off-the-shelf
implementation of GBRT learning algorithm is available in the
Scikit-learn library~\cite{pedregosa2011scikit}.


%We emperically chose it as the learninig model for this task using off-the-shelf implementation from Scikit-learn library \cite{pedregosa2011scikit}. During test time, for a pose hypothesis, we extract its features as we did for the training data and feed into GBRT. GBRT is expected to predict the ADI score for this pose hypothesis, which will then be used to guide the ILP process.  



\emph{B. Features Indicating Good Pose Alignment with Data:} The feature
indicators can be split into two categories:

\begin{myitem}
\item[-] scores evaluating the consistency of the model hypothesis, 
\item[-] scores that reflect the alignment of the scene predictions
(object classes and visible boundaries) with the hypothesis.
\end{myitem}

Given a model $M$ with pose hypothesis $T$, the visible surface
$V(T)$ and visible object boundary $B(T)$ are both computed in the
hypothesis generation process. The mask $S_B$ contains the predicted
boundaries in the RGB image and is generated by setting a threshold
and retaining all pixels $p$ that have $P_B(p)$ higher than the
threshold.  Then, the model consistency scores are given
by:

\begin{myitem}
\item $f_1(T)$ computes the ratio of the pixels in the boundary $B(T)$
induced by pose $T$ that are also in the boundary $S_B$ predicted by
the \cnn: $f_1(T) = \frac{|B(T)\cap S_B|}{|B(T)|},$;
\item $f_2(T)$ computes within the predicted boundary $S_B$ the ratio of the
pixels in the boundary $B(T)$ to the pixels in the visible surface
$V(T)$: $f_2(T) = \frac{|B(T)\cap S_B|}{|V(T) \cap S_B|}$;
\item The third score, $f_3(T)$ computes the percentage of pixels $p$
in $V(T)$ that are well aligned with the depth map: $f_3(T)
= \frac{\sum_{p \in V(T)} \mathbf{1}_{|d(p,T,M) - d(p)|
< \delta_S}}{|V(T)|}$, where $d(p,T,M)$ is the depth of pixel $p$ when
model $M$ is placed according to pose $T$, and $d(p)$ is the depth of
$p$ in the actual depth map.
\end{myitem}

\noindent On the other hand, scene alignment scores are defined as
follows:

\begin{eqnarray*}
&f_4(T) = \sum_{p \in V(T)} P_l(p) \textrm{ \it \small
sim}(p,T,M, \delta_S), \\ &f_5(T) = \sum_{p \in B(T)} (1
- \frac{1}{\delta_B} \textrm{ \it \small dist} (p,S_B, \delta_B)),
\end{eqnarray*}
where: {\small $$\textrm{ \it \small sim}(p,T,M, \delta_S) = (1
- \frac{1}{\delta_S} |d(p,T,M) - d(p)|)(n(p,T,M) \cdot n(p)),$$} and
distances $|d(p,T,M) - d(p)|$ are clipped to $\delta_S$ whenever they
exceed threshold $\delta_S$.  $n(p,T,M)$ is the surface normal of
pixel $p$ when model $M$ is placed according to pose $T$, and $n(p)$
is the surface normal of $p$ in the actual depth map.  $P_l(p)$ is the
probability of label $l$ of the object model in
question. $\textrm{ \it \small dist} (p,S_B, \delta_B)$ computes the
distance between point $p$ and the nearest point to it in the set of
boundaries $S_B$, while limiting the search to a range of $\delta_B$.



==> makefile <==
DOCUMENT  := root

.PHONY: all

TEMPLDIR   := ~/repositories/templates/latex

FORMATDIR  := ../:../format:$(TEMPLDIR)/packages:$(TEMPLDIR)/ieee_format:$(TEMPLDIR)/acm_format:$(TEMPLDIR)/kostas_style:$(TEMPLDIR)/other_format:../$(TEMPLDIR)/ieee_format:../$(TEMPLDIR)/acm_format:../$(TEMPLDIR)/kostas_style:../$(TEMPLDIR)/other_format
FIGUREDIR  := /Users/kb572/repositories/papers/asymp_optimal/ijrr_15/figures/.:.:./figures:../figures:../../figures:../images:../
BIBDIR     := ../:../bib
BINDIR     := ./bin

DVI_OPTIONS := -Ppdf -G0 -tletter
PS2PDF_OPTIONS := -dCompatibilityLevel=1.3 -dMAxSubsetPct=100 -dSubsetFonts=true -dEmbedAllFonts=true -sPAPERSIZE=letter

export TEXINPUTS=.:$(FORMATDIR):$(FIGUREDIR)::
export BIBINPUTS=.:$(BIBDIR):$(FIGUREDIR)::
export BSTINPUTS=.:$(FORMATDIR):$(BIBDIR):$(FIGUREDIR)::

export TEXMFOUTPUT=$(PWD)

latex:
	rubber -v --pdf --warn=all --into $(BINDIR) $(DOCUMENT).tex
	rubber -v --pdf --warn=all --into $(BINDIR) suppl.tex
	rubber -v --pdf --warn=all --into $(BINDIR) rebuttal/response.tex

clean:
	\rm -rf bin/*.out
	rubber --pdf --into $(BINDIR) --clean $(DOCUMENT).tex
	rubber --pdf --into $(BINDIR) --clean suppl.tex


